Inference from modelling the chemodynamical evolution of the Milky Way disc

In this thesis, the field star Initial Mass Function (IMF) and chemical evolution parameters for the Milky Way (MW) are derived using a forward modelling technique in combination with Bayesian statistics. Starting from a local MM disc model, observations of stellar samples in the Solar Neighbourhood are synthesised and compared to the corresponding volume-complete observational samples of Hipparcos stars. The resulting IMF, derived from observations in the range from 0.5 to 8Msun, is a two-slope broken power law with powers of -1.49 +- 0.08 and -3.02 +- 0.06 for the low-mass slope and the high-mass slope, respectively, with a break at 1.39 +- 0.05Msun. In order to constrain the IMF for stars more massive than 8Msun, a fast and flexible chemical enrichment code, Chempy, was developed, which is also able to reproduce spatial and stellar population selections of observational samples. The inferred high-mass slope for stellar masses above 6Msun is -2.28 +- 0.09, accounting for the systematic effects of different yield sets from the literature. This shows that constraints from chemical modelling, similarly to hydrodynamical simulations of the Galaxy, demand a Salpeter high-mass index. This is hard to recover from star count analysis given the rareness of high-mass stars.

==> Chapters/Chapter0A.tex <==
%********************************************************************
% Appendix
%*******************************************************
% If problems with the headers: get headings in appendix etc. right
%\markboth{\spacedlowsmallcaps{Appendix}}{\spacedlowsmallcaps{Appendix}}
\chapter{Appendix Test}
Code from the chemical evolution tool.\\
Which paper or online data were used for the code.\\
The different data sets exploited.\\

==> FrontBackmatter/Declaration.tex <==
%*******************************************************
% Declaration
%*******************************************************
\refstepcounter{dummy}
\pdfbookmark[0]{Declaration}{declaration}
\chapter*{Declaration}
\thispagestyle{empty}
Content of this thesis is available as part of other documents published by the author. Individual sections and illustrations might be very similar and paragraphs may have been reused in exact wording.

\bigskip
This is especially true for:
\begin{itemize}
\item Section III
\end{itemize}
which is extracted from an article on the initial mass function published in MNRAS as part of a paper series \citep{Rybizki2015}.

\bigskip 
\noindent All content of this thesis was compiled and independently written by the author
himself. 
\noindent\textit{\myLocation, \myTime}

\smallskip

\begin{flushright}
    \begin{tabular}{m{5cm}}
        \\ \hline
        \centering\myName \\
    \end{tabular}
\end{flushright}


==> FrontBackmatter/Dedication.tex <==
%*******************************************************
% Dedication
%*******************************************************
\thispagestyle{empty}
%\phantomsection 
\refstepcounter{dummy}
\pdfbookmark[1]{Dedication}{Dedication}

\vspace*{3cm}

\begin{center}
    \emph{Do} I really need a citation? \\
    If yes I might put it here. \\ \medskip
    --- Jan Rybizki    
\end{center}

\medskip

\begin{center}
    Or a dedication. I might put it here.\\ \smallskip
    1985\,--\,2015
\end{center}

==> FrontBackmatter/Foreword.tex <==
\thispagestyle{empty}
%\phantomsection 
\refstepcounter{dummy}
\pdfbookmark[1]{Foreword}{Foreword}

\chapter*{Foreword}
When starting my Ph.D. in astrophysics I followed the fascination which probably everybody experiences when looking into the starred sky on a clear night. In the following years I got the possibility to learn from an international community and indulge on questions closely related to the cycle of matter in the universe. I enjoyed the entertainment coming from satisfying ones thirst for knowledge which might also explain the general public's interest in our field even though its {\it relevance} for people's lives is very limited. Having gone through the process of exploring and contributing to our ken about the Galaxy my focus of interest changed to more earthly topics concerning society and its sustainability. Even though a completely different field I feel well prepared with all the versatile methods and concepts I learned during my degree. Before moving on I want to share my gained insight in this document.\\


==> FrontBackmatter/backup_front/DirtyTitlepage.tex <==
%*******************************************************
% Little Dirty Titlepage
%*******************************************************
\thispagestyle{empty}
%\pdfbookmark[1]{Titel}{title}
%*******************************************************
\begin{center}
    \spacedlowsmallcaps{\myName} \\ \medskip                        

    \begingroup
        \color{Maroon}\spacedallcaps{\myTitle}
    \endgroup
\end{center}        


==> FrontBackmatter/backup_front/Titleback.tex <==
\thispagestyle{empty}

\hfill

\vfill

\noindent\myName: \textit{\myTitle,} \mySubtitle, %\myDegree, 
\textcopyright\ \myTime

\bigskip

\noindent\spacedlowsmallcaps{Supervisors}: \\
\myProf \\
\myOtherProf \\ 
\mySupervisor

\medskip

\noindent\spacedlowsmallcaps{Location}: \\
\myLocation

\medskip

\noindent\spacedlowsmallcaps{Time Frame}: \\
\myTime


==> FrontBackmatter/backup_front/Titlepage.tex <==
%*******************************************************
% Titlepage
%*******************************************************
\begin{titlepage}
	% if you want the titlepage to be centered, uncomment and fine-tune the line below (KOMA classes environment)
	\begin{addmargin}[-1cm]{-3cm}
    \begin{center}
        \large  

        \hfill

        \vfill

        \begingroup
            \color{MidnightBlue}\spacedallcaps{\myTitle} \\ \bigskip
        \endgroup

        \spacedlowsmallcaps{\myName}

        \vfill

        \includegraphics[width=6cm]{gfx/frontpic/figure_2.pdf} \\ \medskip

        \mySubtitle \\ \medskip   
        %\myDegree \\
        %\myDepartment \\                            
        %\myFaculty \\
        %\myUni \\ \bigskip

        \myTime\ -- \myVersion

        \vfill                      

    \end{center}  
  \end{addmargin}       
\end{titlepage}   

==> README <==
A Classic Thesis Style
An Homage to The Elements of Typographic Style
Copyright (C) 2012 Andr\'e Miede http://www.miede.de

Please see the file ClassicThesis.pdf for more information.
Your comments are highly appreciated.

If you like the style then I would appreciate a postcard. My address 
can be found in the file ClassicThesis.pdf. A collection of the 
postcards I received so far is available online at 
http://postcards.miede.de

License:
This program is free software; you can redistribute it and/or modify
it under the terms of the GNU General Public License as published by
the Free Software Foundation; either version 2 of the License, or
(at your option) any later version.

This program is distributed in the hope that it will be useful,
but WITHOUT ANY WARRANTY; without even the implied warranty of
MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
GNU General Public License for more details.

You should have received a copy of the GNU General Public License
along with this program; see the file COPYING.  If not, write to
the Free Software Foundation, Inc., 59 Temple Place - Suite 330,
Boston, MA 02111-1307, USA.

